Local-to-global Perspectives on Graph Neural Networks

This thesis presents a local-to-global perspective on graph neural networks (GNN), the leading architecture to process graph-structured data. After categorizing GNN into local Message Passing Neural Networks (MPNN) and global Graph transformers, we present three pieces of work: 1) study the convergence property of a type of global GNN, Invariant Graph Networks, 2) connect the local MPNN and global Graph Transformer, and 3) use local MPNN for graph coarsening, a standard subroutine used in global modeling.

==> sections/icml-version_arXiv/newproof.tex <==
\convergenceafterEM*

\begin{proof}
Using the triangle inequality
\begin{align*}
& MSE_U(\Phi_c(W), \Phi_d(\hat{W})) \\
& = \|S_U \Phi_c(W)-\frac{1}{n}\Phi_d (\hat{W}) \| \\ 
& = \|S_U \Phi_c(W)- S_U\Phi_c(\inducedW) + S_U\Phi_c(\inducedW) - \Phi_dS_U(\inducedW) + \Phi_dS_U(\inducedW) - \frac{1}{n}\Phi_d (\hat{W})\|\\
&\leq \underbrace{\|S_U \Phi_c(W)- S_U\Phi_c(\inducedW)\|}_\text{First term: discrization error} + 
\underbrace{\|S_U\Phi_c(\inducedW) - \Phi_dS_U(\inducedW)\|}_\text{Second term: sampling error} + \underbrace{\|\Phi_dS_U(\inducedW) - \frac{1}{n}\Phi_d (\hat{W})\|}_\text{Third term: estimation error} \numberthis \label{equ:threeterms} %
\end{align*}
The three terms measures the different sources of error. First term is concerned with the discreization error. Second term concerns the sampling error from randomness of $U$. This term will vanish if we consider only $S_n$ instead of $S_U$.
The third term concerns the edge probablity estimation error.

For the first term $\|S_U \Phi_c(W) - S_U \Phi_c (\inducedW) \| = \| S_U(\Phi_c(W) - \Phi_c(\inducedW))\|$, if suffices to upper bound $\|\Phi_c(W)-\Phi_c(\inducedW)\|_{L_\infty}$ according to property of $S_U$. Since $\| \Phi_c W - \Phi_c \inducedW\|_{L_\infty} \leq C\|W - \inducedW\|_{L_\infty}$ by \Cref{corollary:$k$-IGN-convergence}, and $\|W - \inducedW\|_{L_\infty}$ converges to 0 in probability according to \Cref{lem:inducedW-converges}, we conclude that the first term will converges to 0 with high probability. 


For the third term $\| \Phi_d S_U (\inducedW) - \frac{1}{n}\Phi_d (\hat{W})\| = \| \Phi_d S_U (\inducedW) - \Phi_d (\frac{1}{n}\hat{W})\| $, we know that $\|S_U(\inducedW) -  \frac{1}{n}\hat{W}\|_2 = \frac{1}{n}\|\hat{W}_{n\times n} - W_{n\times n}\|_2 \leq \|\hat{W}_{n\times n} - W_{n\times n}\|_{2, \infty}$, which will also goes to 0 with high probability as $n$ increases according to the statistical guarantee of edge probability estimation of neighborhood smoothing algorithm \citep{zhang2015estimating}, stated in \Cref{thm:graphon-estimation}. Therefore by \Cref{corollary:$k$-IGN-convergence}, the last term also goes to 0 with high probability.   

Therefore the rest work is to control the second term $\|S_U \Phi_c(\inducedW) - \Phi_d S_U(\inducedW)\|$. Again, we use the triangle inequality
\begin{align*}
& \tn{Second term} \\
& = \|S_U \Phi_c(\inducedW) - \Phi_d S_U(\inducedW)\| \\
& \leq \|S_U \Phi_c(\inducedW) - \sampleE \Phi_c(\inducedEW) \| + \| \sampleE \Phi_c(\inducedEW) - \Phi_d S_U(\inducedW)\| \\
& =  \|S_U \Phi_c(\inducedW) - \sampleE \Phi_c(\inducedEW) \| + \| \sampleE \Phi_c(\inducedEW) - \Phi_d \sampleE(\inducedEW)\|\\
& = \|S_U \Phi_c(\inducedW) - \sampleE \Phi_c(\inducedEW) \|\\
& \leq \|S_U \Phi_c(\inducedW) - S_U \Phi_c(\inducedEW)\| + \|S_U \Phi_c(\inducedEW) - \sampleE \Phi_c(\inducedEW)  \| \\
& = \underbrace{\|S_U (\Phi_c \inducedW - \Phi_c \inducedEW)\|}_\text{term $a$} + 
\underbrace{\|(S_U - \sampleE)\Phi_c(\inducedEW) \|}_\text{term $b$}
\end{align*}
The second equality holds because $S_U(\inducedW) = S_n(\inducedEW)$ by definition of $\inducedEW$. The third equality holds because for $\inducedEW$, evaluation operator $S_n$ and linear permutation equivariant $\Phi$ commutes according to \Cref{lem:T-shrinks-L-inf-norm}. 
We will bound the term a) $\|S_U (\Phi_c \inducedW - \Phi_c \inducedEW)\|$ and b) $\|(S_U - \sampleE)\Phi_c(\inducedEW) \|$ next. 

For term a) $\|S_U (\Phi_c \inducedW - \Phi_c \inducedEW)\|$, if suffices to prove that $\|\Phi_c \inducedW -\Phi_c \inducedEW)\|_{L_\infty}$ converges to 0 with high probability. Since $\|\Phi_c \inducedW - \Phi_c \inducedEW)\|_{L_\infty} \leq C\|\inducedW - \inducedEW \|_{L_\infty} \leq C(\|\inducedW - W \|_{L_\infty} + \|\inducedEW - W \|_{L_\infty})$, we only need to upper bound $\|\inducedW - W \|_{L_\infty}$ and $\|\inducedEW - W \|_{L_\infty}$, which are proved by \Cref{lem:inducedW-converges} and \Cref{lem:inducedEW-converges} respectively. 


For term b) $\|(S_U - \sampleE)\Phi_c(\inducedEW) \|$
\begin{align*}
&\|(S_U - \sampleE)\Phi_c(\inducedEW) \| \\
&= \|(S_U \Phi_c(\inducedEW) - \sampleE \Phi_c(\inducedEW)\|\\
& = \|(S_U \Phi_c(\inducedEW) - S_U \Phi_c(W) + S_U \Phi_c(W) - S_n \Phi_c(W) + S_n \Phi_c(W) - \sampleE \Phi_c(\inducedEW)\| \\
& \leq \|(S_U \Phi_c(\inducedEW) - S_U \Phi_c(W) \| + \|S_U \Phi_c(W) - S_n \Phi_c(W)\|  + \|S_n \Phi_c(W) - \sampleE \Phi_c(\inducedEW)\|\\
& \leq \|(S_U (\Phi_c\inducedEW-\Phi_c W) \| + \|S_U \Phi_c(W) - S_n \Phi_c(W)\| + \|\sampleE (\Phi_c\inducedEW-\Phi_c W)\|
\end{align*}
For the first and last term, by the property of $S_U, S_n$ and $\Phi_c$, it suffices to bound $\|W-\inducedEW \|_{L_\infty}$. As $\|W-\inducedEW \|_{L_\infty}$ converges to 0 almost surely (therefore in probablity) by \Cref{lem:inducedEW-converges}, we conclude that the first and last term converges to 0 almost surely. 
For the second term $\|S_U \Phi_c(W) - S_n \Phi_c(W)\|$, it converges to 0 almost surely according to the second part of \Cref{lem:sxsn-sampling}. 



As all terms converge to 0 in the probability or almost surely, we conclude that $\|S_U \Phi_c(W)-\Phi_d (\hat{W}) \|$ converges to 0 in probability.
\end{proof}


==> sections/icml-version_arXiv/oldproof.tex <==
\begin{proof}
Using the triangle inequality
\begin{align*}
& MSE_U(T_c(W), T_d(\hat{W})) \\
& = \|S_U T_c(W)-\frac{1}{n}T_d (\hat{W}) \| \\ 
& = \|S_U T_c(W)- S_UT_c(\inducedW) + S_UT_c(\inducedW) - T_dS_U(\inducedW) + T_dS_U(\inducedW) - \frac{1}{n}T_d (\hat{W})\|\\
&\leq \underbrace{\|S_U T_c(W)- S_UT_c(\inducedW)\|}_\text{First term} + 
\underbrace{\|S_UT_c(\inducedW) - T_dS_U(\inducedW)\|}_\text{Second term} + \underbrace{\|T_dS_U(\inducedW) - \frac{1}{n}T_d (\hat{W})\|}_\text{Third term} %
\end{align*}
The three terms measures the different sources of error. First term is concerned with the discreization error. Second term concerns the sampling error from randomness of $U$. This term will vanish if we consider only $S_n$ instead of $S_U$.
The third term concerns the edge probablity estimation error.

For the first term $\|S_U T_c(W) - S_U T_c (\inducedW) \| = \| S_U(T_c(W) - T_c(\inducedW))\|$, if suffices to upper bound $\|T_c(W)-T_c(\inducedW)\|_{L_\infty}$ according to property of $S_U$. Since $\| T_c (W - \inducedW)\|_{L_\infty} \leq C\|W - \inducedW\|_{L_\infty}$ by \Cref{corollary:$k$-IGN-convergence}, and $\|W - \inducedW\|_{L_\infty}$ converges to 0 in probability according to \Cref{lem:inducedW-converges}, we conclude that the first term will converges to 0 with high probability. Note that \Cref{lem:inducedW-converges} relies on $W$ beling \lip{} and will not hold in later layers. 

\textcolor{blue}{For the first term $\|S_U T_c(W) - S_U T_c (\inducedW) \| = \| S_U(T_c(W) - T_c(\inducedW))\|$, if suffices to upper bound $\|T_c(W)-T_c(\inducedW)\|_{L_2}$ according to NEW property of $S_U$. Since $\| T_c (W - \inducedW)\|_{L_2} \leq C\|W - \inducedW\|_{L_2}$ by \Cref{thm:$2$-IGN-convergence}, and $\|W - \inducedW\|_{L_2}$ converges to 0 in probability according to second part of \Cref{lem:inducedW-converges}. Therefore we conclude that the first term will converges to 0 with high probability. 
}


For the third term $\| T_d S_U (\inducedW) - \frac{1}{n}T_d (\hat{W})\|$, we know that $\|S_U(\inducedW) -  \frac{1}{n}\hat{W}\|_2 = \frac{1}{n}\|\hat{W}_{n\times n} - W_{n\times n}\|_2 \leq \|\hat{W}_{n\times n} - W_{n\times n}\|_{2, \infty}$, which will also goes to 0 with high probability as $n$ increases according to the statistical guarantee of edge probability estimation of neighborhood smoothing algorithm \citep{zhang2015estimating}, stated in \Cref{thm:graphon-estimation}. Therefore by \Cref{corollary:$k$-IGN-convergence}, the last term also goes to 0 with high probability.   

Therefore the rest work is to control the second term $\|S_U T_c(\inducedW) - T_d S_U(\inducedW)\|$. Again, we use the triangle inequality
\begin{align*}
& \tn{Second term} \\
& = \|S_U T_c(\inducedW) - T_d S_U(\inducedW)\| \\
& \leq \|S_U T_c(\inducedW) - \sampleE T_c(\inducedEW) \| + \| \sampleE T_c(\inducedEW) - T_d S_U(\inducedW)\| \\
& =  \|S_U T_c(\inducedW) - \sampleE T_c(\inducedEW) \| + \| \sampleE T_c(\inducedEW) - T_d \sampleE(\inducedEW)\|\\
& = \|S_U T_c(\inducedW) - \sampleE T_c(\inducedEW) \|\\
& \leq \|S_U T_c(\inducedW) - S_U T_c(\inducedEW)\| + \|S_U T_c(\inducedEW) - \sampleE T_c(\inducedEW)  \| \\
& = \underbrace{\|S_U T_c (\inducedW - \inducedEW)\|}_\text{term $a$} + 
\underbrace{\|(S_U - \sampleE)T_c(\inducedEW) \|}_\text{term $b$}
\end{align*}
The second equality holds because $S_U(\inducedW) = S_n(\inducedEW)$. The third equality holds because for $\inducedEW$, evaluation operator $S_n$ and linear permutation equivariant $T$ commutes. 
We will bound the term a) $\|S_U T_c (\inducedW - \inducedEW)\|$ and b) $\|(S_U - \sampleE)T_c(\inducedEW) \|$ next. 

For term a) $\|S_U T_c (\inducedW - \inducedEW)\|$, if suffices to prove that $\|T_c (\inducedW - \inducedEW)\|_{L_\infty}$ converges to 0 with high probability. Since $\|T_c (\inducedW - \inducedEW)\|_{L_\infty} \leq C\|\inducedW - \inducedEW \|_{L_\infty} \leq C|\|\inducedW - W \|_{L_\infty} + \|\inducedEW - W \|_{L_\infty}|$, we only need to bound $\|\inducedW - W \|_{L_\infty}$ and $\|\inducedEW - W \|_{L_\infty}$, which are proved by \Cref{lem:inducedW-converges} and \Cref{lem:inducedEW-converges} respectively. %

\textcolor{blue}{For term a) $\|S_U T_c (\inducedW - \inducedEW)\|$, if suffices to prove that $\|T_c (\inducedW - \inducedEW)\|_{L_2}$ converges to 0 with high probability. Since $\|T_c (\inducedW - \inducedEW)\|_{L_2} \leq C\|\inducedW - \inducedEW \|_{L_2} \leq C|\|\inducedW - W \|_{L_2} + \|\inducedEW - W \|_{L_2}|$, we only need to bound $\|\inducedW - W \|_{L_2}$ and $\|\inducedEW - W \|_{L_2}$, which are proved by \Cref{lem:inducedW-converges} and \Cref{lem:inducedEW-converges} respectively.}


For term b) $\|(S_U - \sampleE)T_c(\inducedEW) \|$
\begin{align*}
&\|(S_U - \sampleE)T_c(\inducedEW) \| \\
&= \|(S_U T_c(\inducedEW) - \sampleE T_c(\inducedEW)\|\\
& = \|(S_U T_c(\inducedEW) - S_U T_c(W) + S_U T_c(W) - S_n T_c(W) + S_n T_c(W) - \sampleE T_c(\inducedEW)\| \\
& \leq \|(S_U T_c(\inducedEW) - S_U T_c(W) \| + \|S_U T_c(W) - S_n T_c(W)\|  + \|S_n T_c(W) - \sampleE T_c(\inducedEW)\|\\
& \leq \|(S_U T_c(\inducedEW-W) \| + \|S_U T_c(W) - S_n T_c(W)\| + \|\sampleE T_c(\inducedEW-W)\|
\end{align*}
For the first and last term, by the property of $S_U, S_n$ and $T_c$, it suffices to bound $\|W-\inducedEW \|_{L_\infty}$. As $\|W-\inducedEW \|_{L_\infty}$ converges to 0 almost surely by \Cref{lem:inducedEW-converges}, we conclude that the first and last term converges to 0 almost surely. 
For the second term $\|S_U T_c(W) - S_n T_c(W)\|$, it converges to 0 almost surely according to second part of \Cref{lem:sxsn-sampling}. 


\textcolor{blue}{For the first and last term, by the property of $S_U, S_n$ and $T_c$, if suffices to bound $\|W-\inducedEW \|_{L_2}$. As $\|W-\inducedEW \|_{L_2}$ converges to 0 almost surely by \Cref{lem:inducedEW-converges}, we conclude that first and last term converges to 0 almost surely. 
For the second term $\|S_U T_c(W) - S_n T_c(W)\|$, it converges to 0 almost surely according to second part of \Cref{lem:sxsn-sampling}.}


As all terms converge to 0 in the probability or almost surely, we conclude that $\|S_U T_c(W)-T_d (\hat{W}) \|$ converges to 0 in probability.
\end{proof}

